Why so? or Why no? Functional Causality for Explaining Query Answers

In this paper, we propose causality as a unified framework to explain query answers and non-answers, thus generalizing and extending several previously proposed approaches of provenance and missing query result explanations. We develop our framework starting from the well-studied definition of actual causes by Halpern and Pearl. After identifying some undesirable characteristics of the original definition, we propose functional causes as a refined definition of causality with several desirable properties. These properties allow us to apply our notion of causality in a database context and apply it uniformly to define the causes of query results and their individual contributions in several ways: (i) we can model both provenance as well as non-answers, (ii) we can define explanations as either data in the input relations or relational operations in a query plan, and (iii) we can give graded degrees of responsibility to individual causes, thus allowing us to rank causes. In particular, our approach allows us to explain contributions to relational aggregate functions and to rank causes according to their respective responsibilities. We give complexity results and describe polynomial algorithms for evaluating causality in tractable cases. Throughout the paper, we illustrate the applicability of our framework with several examples. Overall, we develop in this paper the theoretical foundations of causality theory in a database context.

==> conclusions.tex <==
\section{Conclusions and Future Work} 
\label{sec:conclusions_and_future_work}

In this paper, we defined \emph{functional causes}, a rigorous and extensible definition of causality
encoding the semantics of \emph{causal structures} with the help of powerful \emph{potential functions}. Through theoretical analysis of its properties, we demonstrated that our definition provides a more powerful and robust way to reason about causes than other established notions of causality.
Albeit NP-hard in the general case, common categories of causal networks that correspond to interesting database examples (e.g. safe queries) prove to be tractable.
We presented several database examples that portrayed the applicability of our framework in the context of provenance, explanation of non-answers, as well as aggregates.
We demonstrated how to determine causes of query results for \sqll{SUM} and \sqll{COUNT} aggregates, and how these can be ranked according to the causality metric of \emph{responsibility}.

Overall, with this work we establish the theoretical foundations of causality theory in the database context, which we view as a unified framework that deals with query result explanations. It also brings forth many interesting problems that can be explored in future work. 

This paper focused on deterministic cases; we plan to extend our framework to \emph{probabilistic data} in the future. The fact that functional causes are based on the use of potential functions makes this extension straightforward: the set of Boolean variables $\vec X$ for tuples in the deterministic case becomes a set of probabilities  $\vec x$.
Note that this would not be possible if the causality definition had used just the Boolean formulas.
Potential functions also have the additional advantage that they can be analytically manipulated as opposed to Boolean functions. We currently investigate the properties of their derivatives with the intuition that they reveal another facet of causality, particularly with regard to aggregates and probabilities.

==> relatedWork.tex <==

\section{Related Work}\label{sec:relatedWork}
Our work is mainly related and unifies ideas from three main areas: research on \emph{causality}, \emph{provenance}, and  \emph{missing query result explanations}.

\introparagraph{Causality}
Causality is an active research area mainly in logic and philosophy with their own dedicated workshops (see e.g.\ \cite{CausalityWorkshop:2009}). The most prevalent definitions of causality are based on the idea of \emph{counterfactual causes}, i.e.\ causes are explained in terms of counterfactual conditionals of the form \emph{If $X$ had not occurred, $Y$ would not have occurred}. This idea of counterfactual causality can be traced back to Hume \cite{Menzies:Causation2008}. The best known counterfactual analysis of causation in modern times is due to  Lewis \cite{Lewis1973}. 
In a databases setting, Miklau and Suciu~\cite{DBLP:conf/sigmod/MiklauS04} define \emph{critical tuples} as those which can become counterfactual under some value assignment of variables.
Halpern and Pearl \cite{HalpernPearl:Cause2005} (HP in short) define a variation they call \emph{actual causality}.
Roughly speaking, the idea is that $X$ is a cause of $Y$ if $Y$ counterfactually depends on $X$ under ``some'' \emph{permissive contingency}, where ``some'' is elaborately defined.
Later, Chockler and Halpern \cite{DBLP:journals/jair/ChocklerH04} define the degree of \emph{responsibility} as a gradual way to assign causality.
Eiter and Lukasiewicz \cite{DBLP:journals/ai/EiterL02} show that the problem of detecting whether 
$X = x^0$ is an actual cause of an event is $\Sigma^P_2$-complete for general acyclic models and NP-complete for binary acyclic models. They also give an alleged proof 
showing that actual causality is always reducible to primitive events. However, Halpern \cite{DBLP:conf/kr/Halpern08a} later gives an example for non-primitive actual causes, showing this proof to ignore some cases under the original definition. Chockler et al.~\cite{DBLP:journals/tocl/ChocklerHK08} later apply causality and responsibility to binary Boolean networks, giving a modified definition of cause which, as we show in \autoref{appendix:DiscussionCHK}, introduces new counter-intuitive problems and, despite claims to be otherwise, is \emph{not equal} to the original HP definition of actual cause.

Our definition of \emph{functional cause} builds upon the HP definition, but extends it with several desirable properties:  causes are \emph{always} primitive input variables, network expansion cannot create new causes, and the definition fixes intuitive examples where the HP-definition does not follow consensus in the causality literature. 
It is these properties that allow us to apply our causality framework to a database setting in \autoref{sec:explaining_query_results}.





\introparagraph{Provenance}
Approaches for defining data provenance can be mainly divided into three categories: 
\emph{how}, \emph{why}, and \emph{where} provenance 
\cite{DBLP:conf/icdt/BunemanKT01, DBLP:journals/ftdb/CheneyCT09, DBLP:journals/tods/CuiWW00, DBLP:conf/pods/GreenKT07}.
In particular for the ``why so'' case, we observe a close connection between 
provenance and causality, where it is often the case that tuples in the 
provenance for the result of a positive query result are causes.
While none of the work on provenance mentions or makes direct connections
to causality, those connections can be found.
The work by Buneman et al.\ \cite{DBLP:conf/icdt/BunemanKT01} makes a 
distinction between why and where provenance that can be connected to 
causality as follows: 
\emph{why provenance} returns all tuples that can be considered
causes for a particular result, and \emph{where provenance} 
returns attributes along a particular causal path. 
Green et al.\ \cite{DBLP:conf/pods/GreenKT07} present a generalization
for all types of provenance as semirings; finding functional causes in a Boolean tree, if taken in a provenance context,  yields degree-one polynomials for provenance semirings. 
View data lineage, as presented by Cui et al.\ \cite{DBLP:journals/tods/CuiWW00}
also addresses aggregates but lacks a notion of graded contribution and returns all tuples
that contribute to an aggregate.

In contrast, our approach can rank tuples according to their \emph{responsibility}, hence our approach allows to determine a gradual contribution with counterfactual tuples ranked first. Also,
in contrast to our paper, most of the work on provenance has little or no 
connection to the philosophical groundwork on causality.
We take this work and significantly adapt it so that it can be applied to databases. 








\introparagraph{Missing query results}
Very recent work has focused on the question ``why no'', i.e.\ why is 
a certain tuple {\em{not}} in the result set?
The work by Huang et al. \cite{DBLP:journals/pvldb/HuangCDN08} 
presents provenance for potential answers and 
never answers.  In 
the case that no insertions or modifications can yield the desired result - 
usually for privacy or security reasons -  
the system declares that particular tuple a never answer.  
Both Huang's work and Artemis  \cite{DBLP:journals/pvldb/HerschelHT09}
handle potential answers by providing
tuple insertions or modifications that would yield the missing
tuples.  Alternatively, 
Chapman and Jagadish \cite{DBLP:conf/sigmod/ChapmanJ09} focus
on which \emph{manipulation} in the query plan  
eliminated a specific tuple.  
Lim et al.\ \cite{DBLP:conf/chi/LimDA09} adopt a third, 
explanation-based, approach.  This approach aims to answer questions such
as {\em{why, why not, how to,}} and {\em{what if}} for context-aware 
applications, but does not address a database setting.

Our work, unifies the above approaches in the sense that we model both, \emph{tuples} or \emph{manipulations} as possible causes for missing query answers. Also, our approach unifies the problem of explaining missing query answers 
(\emph{why} is a tuple not in the query result) with work on provenance (\emph{why} is a tuple in the query result).


\introparagraph{Other}
Minsky and Papert initiated the study of the computational properties of Boolean functions using
their representation by polynomials and call this the \emph{arithmetic} instead of the logical form~\cite[p.27]{MinskyPapert1987:Perceptrons}. This method was later successfully used in complexity theory and became known as \emph{arithmetization}~\cite{DBLP:journals/cc/BabaiF91}.






